ORPHEUS: Living Labs for End-to-End Data Infrastructures for Digital Agriculture

IoT networks are being used to collect, analyze, and utilize sensor data. There are still some key requirements to leverage IoT networks in digital agriculture, e.g., design and deployment of energy saving and ruggedized sensor nodes (SN), reliable and long-range wireless network connectivity, end-to-end data collection pipelines for batch and streaming data. Thus, we introduce our living lab ORPHEUS and its design and implementation trajectory to showcase our orchestrated testbed of IoT sensors, data connectivity, database orchestration, and visualization dashboard. We deploy light-weight energy saving SNs in the field to collect data, using LoRa (Long Range wireless) to transmit data from the SNs to the Gateway node, upload all the data to the database server, and finally visualize the data. For future exploration, we also built a testbed of embedded devices using four different variants of NVIDIA Jetson development modules (Nano, TX2, Xavier NX, AGX Xavier) to benchmark the potential upgrade choices for SNs in ORPHEUS. Based on our deployment in multiple farms in a 3-county region around Purdue University, and on the Purdue University campus, we present analyses from our living lab deployment and additional components of the next-generation IoT farm.

==> 10-looking-ahead.tex <==
\section{Looking Ahead}
\label{sec:looking-ahead}
\noindent Big data and precision agriculture will likely be a disruptive force in the farm economy over the medium to long-term range. Digital agriculture, with the incorporation of IoT-based technologies, presents the ability to evaluate a system at multiple levels (individual, local, regional, and global) and generate tools that allow for improved decision making in every sub-process related to digital agriculture. %In this article, we have reviewed the different types of datasets and relevant data science processing algorithms in typical field operations together with thoughts on the typical lifecycle for the data to be contributory to the digital farm economy. We have then discussed storage and fast information-retrieval solutions. Then, we have adapted some core Machine Learning concepts to digital agriculture, which means putting domain-specific requirements regarding interpretability, distribution, ability to handle intermittent wireless connectivity, and low cost. Finally, we have instantiated the framework into a cloud computing environment for long-term storage, analysis, and visualization. 
% Finally, we have developed the theme of machine learning and cloud computing for agriculturists by instantiating and implementing open-source data processing frameworks. We conclude by discussing analytics for alternative agriculture for generation of biofuels and policy challenges of the implementation of digital agriculture approaches in the wild. 

% Technological advancements have led to farm consolidation in the past. Newer and more efficient tools reduce per-unit costs, allowing small and mid-size farms to become more profitable and therefore more prevalent. Moreover, economies of scale---the ability of large firms to spread investment costs over many units of production---allow large operations to exploit precision agriculture and big data tools earlier, potentially accelerating the consolidation trend~\cite{coble2016advancing}. As mechanization continues and farm operations become more digitized, their labor needs will reduce and will become specialized. This could mitigate the so-called ``brain drain'' impacting many rural communities in the U.S.~\cite{artz2003brain}. 
\begin{comment}
An important focus of the paper is on the convergence of IoT and ML on the one side and agricultural sustainability on the other. The ability to track virtually every farm activity through ubiquitous and inexpensive sensors has spurred efforts to increase sustainability and can be verified and certified by third-parties. 
% For example, Indigo Ag, a digital agriculture startup, is attempting 
For example, there are already commercial efforts to monetize on-farm carbon sequestration for farms using regenerative practices~\cite{indigoag}. Blockchain technology promises to increase sustainability and ensure food safety by authenticating information across the food system~\cite{nagaraj2019panel}. In additional to privacy concerns, adoption of precision agriculture and big data is limited by the availability of broadband internet in rural areas~\cite{whitacre2014connected}. Thus, looking at the policy angle, integrated farm equipment and sensors pipe data up to the cloud in real time meaning farmers are more reliant on upload speeds than the typical user. The societal returns to rural broadband are large though immediate private gains are often unclear. This suggests that high-speed internet will be under-supplied in the market and stresses a role for governmental support. This has been argued by federal government sources like USDA~\cite{usda-broadband-2019} as well state government sources, such as in Indiana~\cite{grant2018broadband}. 
\end{comment}
% Old conclusion
\begin{comment}
\noindent Big data and precision agriculture will likely be a disruptive force in the farm economy over the medium to long-term. Technological advancements have led to farm consolidation in the past. Newer and more efficient tools reduce per-unit costs, allowing small and mid-size farms to become more profitable and therefore more prevalent. Moreover, economies of scale---the ability of large firms to spread investment costs over many units of production---allow large operations to exploit precision agriculture and big data tools earlier, potentially accelerating the consolidation trend~\cite{coble2016advancing}. As mechanization continues and farm operations become more digitized, their labor needs will reduce and will become specialized. This could mitigate the so-called ``brain drain'' impacting many rural communities in the U.S.~\cite{artz2003brain}. 

The ability to track virtually every farm activity through ubiquitous and inexpensive sensors means that efforts to increase sustainability can be verified and certified by third-parties. 
% For example, Indigo Ag, a digital agriculture startup, is attempting 
For example, there are already commercial efforts to monetize on-farm carbon sequestration for farms using regenerative practices~\cite{indigoag}. Blockchain technology promises to increase sustainability and ensure food safety by authenticating information across the food system. In additional to privacy concerns, adoption of precision agriculture and big data is limited by the availability of broadband internet in rural areas~\cite{whitacre2014connected}. Integrated farm equipment and sensors pipe data up to the cloud in real time meaning farmers are more reliant on upload speeds than the typical user. The societal returns to rural broadband are large though immediate private gains are often unclear. This suggests that high-speed internet will be under-supplied in the market and implying a role for external support. This has been argued by federal government sources like USDA~\cite{usda-broadband-2019} as well state government sources, such as in Indiana~\cite{grant2018broadband}. 
\end{comment}

==> 6-democratizing-AI.tex <==
\section{Democratizing AI for Farmers}
%SC: incorporated relevant stuff from this section in the conclusion. removed this section.
\label{sec:democratizing-ai}
\noindent This will require the accessibility of state-of-the-art wireless, database, and ML technologies to farms---even small-scale farms---deploying leading-edge analytics and broadband modalities to gather data from farms (\eg FarmBeats, AirBand technologies, Open Ag Data Alliance APIs). %For example, in Fig.~\ref{fig:analytics-arch}, these is deployed on the compute server and customized to the kinds of data and the analytics for digital agriculture. 
This will cover the commercial angle of deploying and operating a system and the foundational (and often open-source) technologies that they build upon, such as, TV whitespace spectrum being used to upload high volume data.
To bring the benefits of digital agriculture, and the ML driven insights to the farmers, we need to make these systems
affordable. However, existing digital agriculture solutions are expensive for two key reasons. 

\underline{First}, is the limited broadband connectivity in rural farms. The sensors, drones, and tractors need to send data to the
cloud to train the ML models, and the insights need to be conveyed to
the farmer's devices. Even in the US, around 20 million rural Americans
do not have broadband access~\cite{fc2019eighth}. And a large part of
farmland does not have access either.
%https://www.fcc.gov/reports-research/reports/broadband-progress-reports/eighth-broadband-progress-report
To bridge this digital divide, we need to come up with innovative
solutions to bring broadband Internet in the farms. One such promising
technology is the TV White Spaces technology, which refers to unused TV
channels~\cite{bahl2009white}. There is abundant unused TV channels in
farms, which can be used to send and receive data in farms. Wireless
signals also propagate smoothly in the TV frequencies, and are ideal for connecting farms. Satellite-based Internet access also holds promise, where low-earth orbit (LEO) satellites could enable low-cost backhaul connectivity.

\underline{Second}, the reason for expensive digital agriculture solutions is the lack of platforms for innovation that are opensource and interoperable. Data acquisition
systems are proprietary, and hence getting data from the farm for research is not easy. There is also a dearth of clean data from farms that can be used for building ML models. 
We propose the building of open-source APIs, and data
repositories. These APIs, such as the one from Open Ag Data Alliance,
afford researchers and startups a platform to prototype their
innovation. Similarly, a cloud-based data repository, for example with
drone imagery and satellite data from research farms, will enable
researchers to train new models. It will also create a
benchmarking dataset to evaluate new innovations before
bringing it to the growers. 


==> 7-limitations.tex <==
\section{Limitations}
%redundant stuff, SC -- removed
\label{sec:limitation}
\noindent{Here we acknowledge the key limitations of our initial work setting up practical testbeds:}
\begin{itemize}
    \item Our solution still needs human intervention such as replacing batteries for SN, and stable power supply for LoRa gateways, which limit the places where we can deploy them.
    \item The bandwidth of LoRa is relatively low such that we cannot transmit complex data (\eg image data, audio data). We can also use 4G and 5G here to transmit data from the SNs to the gateway because they have broader bandwidth, better suited for video feeds, sound feeds, and images.
    \item We need to deploy and maintain our own LoRa and LoRaWAN gateway, which could be quite expensive in short-term. NB-IoT could be a alternative choice, but NB-IoT will have a monthly payment. 
    \somali{put some specifics, what are the plans like -- data volumes to prices and for which vendors, otherwise this is not suitable to put in technical writing}.
    %Depending on whether the task is short-term or long-term, we need to do a trade-off between them. NB-IoT is more suitable for short-term tasks because the one-time payment is quite low. While LoRa is more suitable for long-terms tasks, we don't have monthly payment but the one-time payment will be quite high.
\end{itemize}

==> 8-conclusion-old.tex <==
\section{Conclusion and Future Work}
%SC: don't use this, this is the old conclusion, I rewrote the new one in a separate .tex file [conclusion.tex]
\label{sec:conclusion}
We have built a low-energy, durable, flexible, long-range, low-cost IoT Network. And have inclusive implementation and troubleshooting examples.
For future work, we are aiming to develop smart, self-maintainable, sustainable sensor devices and network.

% \edgardo{Regarding the low-cost benefit, is there a way to show a comparison or support this assertion?}
% \pengcheng{two ways to support this: 1. The traditional agriculture measurements are done by manually work, which include the cost of time, human efforts, and other accessory cost. 2. We give an estimate overall cost of deploying a network in a single farm, and compare it with other solution. The second one may be difficult because we need to find more data.}

\noindent{\customsec{Smart and Sustainable Node \& Gateway}}
\begin{itemize}
    \item Problem: Currently, the SNs need to be powered by batteries. The Gateway can only be put somewhere where have a power supply and Internet access. And need a quite much effort to maintain them.
    \item Our solution: The overall feature of our solution is that they don’t need any human evolving works after the first time deployment. Since the number of IoT devices and networks will explode in the future, sustainable devices and networks is a good point we can emphasize. 
    \item Indesign node + Solar panel (The Indesign node is powered by 4 AAA batteries now, if we can replace the batteries with a solar panel, then we don’t need to go to the field to replace the batteries manually.)
    \item Raspberry-Pi + Solar panel + Camera to serve as a camera SN in the field to do object detection. The detection target could be saboteurs, animals, diseases of crops, or if the height of crops is in anticipation. The traditional camera does not have the ability to analyze the video in the field and needs quite larger network bandwidth to upload the video to the cloud which is very power consuming. By using our method, we can collect the data in the field and directly analyze the video in the field, and only send the results back to the cloud. Since we will have limited power by using the solar panel, we can also incorporate approximate calculation here to save power. And for agriculture application, latency should not be a problem, 5 frames per second should be enough.
    \item A drone carrying Jetson Nano to do object detection. After the drone collected all the data, it can send the data to the Edge Server (a more powerful machine could be Xavier NX
\end{itemize}

\textbf{Improvement on Network:}
\begin{itemize}
    \item Expand longer coverage by combining LoRa and NB-IoT on a single Raspberry-Pi (It will serve as a relay station between SNs and NB-IoT base station, and this is to solve the coverage issue)
    \item An intelligent offloading scheme on the Gateway. We can do data analysis on the Raspberry-Pi directly and only send back the result to the cloud (decreasing the data need to be upload to the cloud).
\end{itemize}







==> 8-discussion.tex <==
\section{Discussion}
\label{sec:discussion}
Here are some valuable experiences we have learned from the deployment of \name:
\begin{itemize}
    \item Since we are using electronic devices to build an IoT network, ruggedizing them to operate outdoors in agriculture settings is vital. Besides, robust firmware to support these devices is also critical. What's more, higher-compute gateway nodes and a backend database server with an in-memory database and application server (\eg Redis), and ability to offload from the SNs or gateway nodes to the cloud-hosted databases is required~\cite{chaterji2021lattice, jiang2020hybrid, chaterji2020cloud}. Such cloud-hosted databases can serve to aggregate the data from multiple farms, and within each farm, from multiple SNs.
    \item When we build the whole end-to-end data collecting and visualization pipeline, data transmission and storage are important. Setting up multiple anchor points in the pipeline will be a good solution to avoid missing data and data tampering. This is accomplished by storing our data in both the gateway nodes and backend servers for groundtruthing and online updates. % of these groundtruth datasets. 
    Further, daily connectivity, and data integrity checks need to be performed to  ensure resiliency of the workflow loop. %And we do daily network connection and data integrity checking on the server.
    \item When building a large-scale IoT network architecture, modular design is a good approach, which allows one to divide the system into discrete scalable and reusable modules. %Flexibility and cost reduction are some of the advantages of a modular design, in order to troubleshoot parts of a large-scale network with minimum downtime. 
    In our living lab, the SNs are designed by following the LoRa protocol so that the wireless communication in the field is done by using LoRa, the Raspberry Pi, and LoStik module serving as the Gateway. Raspberry Pi can potentially be replaced by more powerful devices, \eg Jetsons, at the gateway. %The Raspberry-Pi is not capable enough to do the heavyweight computation, such as, anomaly detection on the sensor data stream (\eg temperature or soil moisture content). 
    The Jetson-class devices can do the heavyweight computation, such as, computing a frequency spectrum of the values and identifying anomalies from them. 
        % Another architecture that we have deployed is that the communication gateway is placed close to the sensors, the sources of data. Then, if the sensors generate high-bandwidth streams, like video, the gateway node equipped with NVIDIA mobile GPU, can run analytics or aggregation on the raw sensor data. Then the gateway only sends the summarized results of the aggregation or the analytics over the LoRa network. This architecture is more efficient because transmitting the result of the object recognition is a lot less data than the raw video stream feeds.
    % PW: commented because it is more like future work
    
   Next, we use standard TCP/IP protocol connecting the Gateway to the Internet. Finally, our website is developed using the Django framework. MongoDB stores all of the data, and acts as an interface between the cloud website, and the edge LPWAN.
    \item This is a real-world implementation work, which is subjected to drastic weather and frequently shifting landscape, affecting wireless communication performance, \eg the height of the corn stalks in a corn field can reduce the packet reception ratio between the SNs and the Gateway. 
    % In our scheme, we use IP67 packages to protect the SNs. Our observations show that the SN can tolerate a temperature as low as -25°C, and relative humidity (RH) as high as 99\%. Based on the consideration of wireless propagation channel model in rural areas, we adopt antenna extension for the SNs, which could greatly improve the received power of the LoRa signal.
    \end{itemize}
